Training Vision Models for LLM-Driven Weight-Space Programming

It has been demonstrated that, in certain settings, large language models can perform weight-space programming to directly modify the weights of neural networks. However, it is unknown how dedicated training of these networks can contribute to the successes of weight-space programming. We present a benchmark of LLM-driven weight-space programming on vision models, in which five LLMs edit convolutional networks and vision transformers on relabeling and error-correction tasks on Waterbirds, CIFAR-100, PACS and Entity-30. We report more than 2,600 such edit processes, whereby each edit is scored on held-out images for success, side effects and accuracy loss. We compare standard training with label smoothing, gradient-based editable training, and our Edit-Ready Training (ERT), a novel method that rehearses the direct, closed-form weight edits LLMs perform. We show that preparing networks for editing raises the success of LLM edits substantially where standard networks are hard to edit. ERT further achieves the highest mean score for GPT-6 Astra and Claude Opus 5.5 across all evaluated baselines. We will release our LLM testing framework alongside all tasks, editing trajectories and scores. Project page: https://viscom.uni-ulm.de/wsp

==> ert-paper-arxiv/bench_preamble.tex <==
\usepackage[T1]{fontenc}
\usepackage{graphicx}
\usepackage{amsmath,amssymb}
\usepackage{booktabs}
\usepackage{microtype}
\usepackage{multirow}
\usepackage{colortbl}
\usepackage{tikz}
\usepackage{wrapfig}
\usetikzlibrary{arrows.meta,positioning}
\definecolor{bestbg}{rgb}{0.84,0.93,0.93}
\newcommand{\best}[1]{\cellcolor{bestbg}#1}
\newcommand{\editorlogo}[1]{\IfFileExists{fig_bench/logo_#1.png}{\raisebox{-0.18em}{\includegraphics[height=0.95em]{fig_bench/logo_#1.png}}}{}}
\newcommand{\cistack}[2]{\begin{tabular}[c]{@{}c@{}}#1\\[-3.5pt]{\fontsize{5.5}{6.5}\selectfont\color{black!55}[#2]}\end{tabular}}
\newcommand{\metricci}[3]{\cistack{#1}{#2,\,#3}}
\newcommand{\bestmetricci}[3]{\cistack{\textbf{#1}}{#2,\,#3}}
\newcommand{\secondmetricci}[3]{\cistack{\underline{#1}}{#2,\,#3}}
\definecolor{deltapos}{rgb}{0.00,0.45,0.25}
\definecolor{deltaneg}{rgb}{0.75,0.10,0.10}
\newcommand{\posdelta}[1]{\textcolor{deltapos}{#1}}
\newcommand{\negdelta}[1]{\textcolor{deltaneg}{#1}}
\newcommand{\sigposdelta}[1]{\textcolor{deltapos}{\boldmath\textbf{#1}}}
\newcommand{\signegdelta}[1]{\textcolor{deltaneg}{\boldmath\textbf{#1}}}
\newcommand{\neudelta}[1]{\textcolor{black!55}{#1}}


==> ert-paper-arxiv/tables_bench/ablation_edits.tex <==
\begin{tabular}{@{}lcccc@{}}
\toprule
Rehearsed edit & Net & $\Delta$ & Pairs $>0$ & $p$ \\
\midrule
\multicolumn{5}{@{}l}{\emph{One training seed, 8 species}} \\
ERT (reference) & 0.72 & & & \\
\quad + bias compensation & 0.76 & $+0.04$ & 4/8 & 0.55 \\
\quad 32 units instead of 8 & 0.76 & $+0.03$ & 4/8 & 0.51 \\
\quad 8 to 64 units, drawn per episode & 0.68 & $-0.04$ & 2/8 & 0.62 \\
\quad step size $\times$1 to 3 & 0.66 & $-0.06$ & 2/8 & 0.26 \\
\quad + agent-shaped edits, combined & 0.75 & $+0.02$ & 3/8 & 0.62 \\
\midrule
\multicolumn{5}{@{}l}{\emph{Two training seeds, 16 pairs}} \\
ERT (reference) & 0.68 & & & \\
\quad stronger rehearsal & 0.73 & $+0.06$ & 10/16 & 0.20 \\
\quad + gradient-step edit & 0.69 & $+0.01$ & 9/16 & 0.79 \\
\bottomrule
\end{tabular}


==> ert-paper-arxiv/tables_bench/ablation_edits_settings.tex <==
\begin{tabular}{@{}lllccccc@{}}
\toprule
Task & Dataset & Network & Pairs & ERT & Variant & $\Delta$ & $p$ \\
\midrule
\multicolumn{8}{@{}l}{\emph{Stronger rehearsal (16 episodes, 64 units, two support images)}} \\
Relabel & Waterbirds & ResNet-18 & 16 & 0.68 & 0.73 & $+0.06$ & 0.20 \\
Relabel & Waterbirds & ViT-B/16 & 8 & 0.82 & 0.76 & $-0.06$ & 0.38 \\
Relabel & CIFAR-100 & ResNet-18 & 8 & 0.67 & 0.61 & $-0.07$ & 0.47 \\
Relabel & CIFAR-100 & ViT-B/16 & 8 & 0.86 & 0.88 & $+0.02$ & 0.58 \\
Confusion fix & CIFAR-100 & ResNet-18 & 8 & 0.61 & 0.51 & $-0.10$ & 0.20 \\
Confusion fix & CIFAR-100 & ViT-B/16 & 8 & 0.74 & 0.69 & $-0.05$ & 0.76 \\
Subgroup fix & PACS & ResNet-18 & 8 & 0.70 & 0.77 & $+0.07$ & 0.02 \\
Subgroup fix & PACS & ViT-B/16 & 8 & 0.80 & 0.66 & $-0.14$ & 0.13 \\
\multicolumn{6}{@{}l}{Mean over settings} & $-0.03$ & \\
\midrule
\multicolumn{8}{@{}l}{\emph{Signed sparse edit instead of the top-8 rule}} \\
Relabel & Waterbirds & ViT-B/16 & 8 & 0.82 & 0.81 & $-0.01$ & 0.75 \\
Relabel & CIFAR-100 & ViT-B/16 & 8 & 0.86 & 0.89 & $+0.03$ & 0.34 \\
\bottomrule
\end{tabular}


==> ert-paper-arxiv/tables_bench/detail_opus.tex <==
Waterbirds relabel, ResNet-18 & 0.51 & 0.101 & $-5.1$ & 87.5 & 0.62 & 0.144 & $-6.0$ & 84.7 & 0.63 & 0.109 & $-7.0$ & 91.4 & 0.73 & 0.107 & $-6.3$ & 91.4 \\
Waterbirds relabel, ViT-B/16 & 0.39 & 0.059 & $-3.8$ & 87.5 & 0.72 & 0.099 & $-5.5$ & 89.1 & 0.87 & 0.081 & $-5.6$ & 93.2 & 0.85 & 0.085 & $-6.5$ & 93.2 \\
CIFAR-100 relabel, ResNet-18 & 0.71 & 0.035 & $-2.8$ & 86.9 & 0.85 & 0.050 & $-4.0$ & 87.6 & 0.71 & 0.050 & $-4.2$ & 87.4 & 0.72 & 0.046 & $-4.0$ & 85.7 \\
CIFAR-100 relabel, ViT-B/16 & 0.84 & 0.029 & $-3.0$ & 93.1 & 0.84 & 0.027 & $-3.1$ & 93.4 & 0.94 & 0.027 & $-3.2$ & 93.5 & 0.88 & 0.020 & $-2.4$ & 93.0 \\
CIFAR-100 confusion fix, ResNet-18 & 0.61 & 0.014 & $-0.8$ & 86.9 & 0.50 & 0.016 & $-1.1$ & 87.7 & 0.63 & 0.026 & $-1.8$ & 87.4 & 0.64 & 0.024 & $-1.5$ & 85.7 \\
CIFAR-100 confusion fix, ViT-B/16 & 0.62 & 0.004 & $-0.2$ & -- & 0.64 & 0.006 & $-0.3$ & -- & 0.72 & 0.006 & $-0.4$ & -- & 0.74 & 0.005 & $-0.2$ & -- \\
Entity-30 confusion fix, ResNet-50 & 0.45 & 0.014 & $-1.0$ & 91.2 & 0.53 & 0.019 & $-1.9$ & 91.5 & 0.61 & 0.015 & $-1.0$ & 91.2 & 0.77 & 0.032 & $-2.4$ & 90.7 \\
PACS subgroup fix, ResNet-18 & 0.78 & 0.057 & $-3.4$ & 88.6 & 0.82 & 0.081 & $-5.1$ & 88.3 & 0.83 & 0.110 & $-7.2$ & 86.9 & 0.79 & 0.088 & $-5.4$ & 86.9 \\
PACS subgroup fix, ViT-B/16 & 0.88 & 0.070 & $-4.1$ & 90.0 & 0.84 & 0.069 & $-4.1$ & 90.0 & 0.71 & 0.063 & $-3.8$ & 89.0 & 0.91 & 0.110 & $-6.6$ & 85.0 \\


==> ert-paper-arxiv/tables_bench/edit_heatmap_stats.tex <==
\begin{tabular}{@{}l rr rrr rrr rrr r@{}}
\toprule
 & & & \multicolumn{3}{c}{Edited units} & \multicolumn{3}{c}{Change of a unit} & \multicolumn{3}{c}{Change of the head} & \\
\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}
 & Edits & Head & min & mean & max & min & mean & max & min & mean & max & Outside \\
\midrule
\multicolumn{13}{@{}l}{\emph{ResNet-18} (512 units)} \\
\quad Opus & 144 & 142 & 1 & 20 & 75 & $2\cdot10^{-7}$ & 0.39 & 22.1 & 0.19 & 2.15 & 22.2 & 13 \\
\quad Astra & 128 & 128 & 1 & 206 & 512 & $1\cdot10^{-7}$ & 0.05 & 10.2 & 0.13 & 1.53 & 17.7 & 4 \\
\quad Gemma & 125 & 63 & 1 & 47 & 512 & $2\cdot10^{-6}$ & 0.16 & 7.07 & 0.08 & 1.98 & 10.1 & 1 \\
\quad GLM & 126 & 107 & 1 & 37 & 512 & $2\cdot10^{-7}$ & 0.12 & 8.00 & $9\cdot10^{-5}$ & 1.14 & 11.3 & 3 \\
\quad DeepSeek & 119 & 118 & 3 & 35 & 94 & $5\cdot10^{-7}$ & 0.12 & 2.00 & 0.09 & 0.85 & 6.82 & 0 \\
\quad all editors & 642 & 558 & 1 & 72 & 512 & $1\cdot10^{-7}$ & 0.10 & 22.1 & $9\cdot10^{-5}$ & 1.52 & 22.2 & 21 \\
\midrule
\multicolumn{13}{@{}l}{\emph{ResNet-50} (2048 units)} \\
\quad Opus & 36 & 33 & 8 & 36 & 142 & $1\cdot10^{-7}$ & 1.43 & 15.1 & 2.51 & 9.97 & 39.0 & 0 \\
\quad Astra & 36 & 35 & 1 & 373 & 2048 & $6\cdot10^{-6}$ & 0.21 & 400 & 0.74 & 21.6 & 400 & 0 \\
\quad all editors & 72 & 68 & 1 & 210 & 2048 & $1\cdot10^{-7}$ & 0.31 & 400 & 0.74 & 15.9 & 400 & 0 \\
\midrule
\multicolumn{13}{@{}l}{\emph{ViT} (768 units)} \\
\quad Opus & 128 & 121 & 2 & 71 & 768 & $3\cdot10^{-5}$ & 0.13 & 2.50 & 0.31 & 1.50 & 7.03 & 1 \\
\quad Astra & 128 & 128 & 51 & 638 & 768 & $2\cdot10^{-7}$ & 0.03 & 1.01 & 0.18 & 0.98 & 3.55 & 0 \\
\quad Gemma & 126 & 52 & 1 & 300 & 768 & $1\cdot10^{-5}$ & 8.65 & 653 & 0.38 & 116 & 5693 & 0 \\
\quad GLM & 125 & 87 & 1 & 127 & 768 & $2\cdot10^{-5}$ & 0.15 & 39.7 & 0.09 & 3.61 & 39.7 & 3 \\
\quad DeepSeek & 126 & 100 & 11 & 122 & 768 & $3\cdot10^{-6}$ & 0.11 & 4.81 & 0.18 & 1.66 & 16.0 & 0 \\
\quad all editors & 633 & 488 & 1 & 265 & 768 & $2\cdot10^{-7}$ & 1.09 & 653 & 0.09 & 14.0 & 5693 & 4 \\
\midrule
\multicolumn{13}{@{}l}{\emph{Training method} (all backbones and editors)} \\
\quad ERM & 335 & 284 & 1 & 165 & 768 & $1\cdot10^{-7}$ & 0.12 & 22.1 & 0.15 & 3.04 & 24.3 & 7 \\
\quad LS & 333 & 270 & 1 & 166 & 768 & $2\cdot10^{-7}$ & 0.06 & 5.32 & 0.06 & 1.28 & 14.0 & 5 \\
\quad ENN & 340 & 279 & 1 & 165 & 2048 & $5\cdot10^{-7}$ & 2.91 & 653 & 0.12 & 22.4 & 5693 & 10 \\
\quad ERT & 339 & 281 & 1 & 164 & 2048 & $2\cdot10^{-6}$ & 0.17 & 400 & $9\cdot10^{-5}$ & 4.67 & 400 & 3 \\
\bottomrule
\end{tabular}


==> ert-paper-arxiv/tables_bench/ert_vs_enn.tex <==
Waterbirds relabel, ResNet-18 & $+0.10$ & 10/16 & 0.043 \\
Waterbirds relabel, ViT-B/16 & $-0.02$ & 4/8 & 0.414 \\
CIFAR-100 relabel, ResNet-18 & $+0.02$ & 4/8 & 0.805 \\
CIFAR-100 relabel, ViT-B/16 & $-0.05$ & 2/8 & 0.062 \\
CIFAR-100 confusion fix, ResNet-18 & $+0.01$ & 5/8 & 0.820 \\
CIFAR-100 confusion fix, ViT-B/16 & $+0.03$ & 4/8 & 0.719 \\
Entity-30 confusion fix, ResNet-50 & $+0.14$ & 7/9 & 0.227 \\
PACS subgroup fix, ResNet-18 & $-0.01$ & 4/8 & 0.812 \\
PACS subgroup fix, ViT-B/16 & $+0.15$ & 7/8 & 0.078 \\


==> ert-paper-arxiv/tables_bench/table1.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}c@{\hspace{3pt}}l*{10}{c}@{}}
\toprule
& & \multicolumn{4}{c}{\textbf{Relabel}} & \multicolumn{3}{c}{\textbf{Confusion fix}} & \multicolumn{2}{c}{\textbf{Subgroup fix}} & \\
\cmidrule(lr){3-6}\cmidrule(lr){7-9}\cmidrule(lr){10-11}
 &
  & \textbf{WB}
  & \textbf{WB}
  & \textbf{C100}
  & \textbf{C100}
  & \textbf{C100}
  & \textbf{C100}
  & \textbf{E30}
  & \textbf{PACS}
  & \textbf{PACS}
  & \\[-0.2em]
& \textbf{Method}
  & \textbf{R18}
  & \textbf{ViT}
  & \textbf{R18}
  & \textbf{ViT}
  & \textbf{R18}
  & \textbf{ViT}
  & \textbf{R50}
  & \textbf{R18}
  & \textbf{ViT}
  & \textbf{Mean} \\
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{\footnotesize\editorlogo{openai}\,\textit{GPT-6 Astra}}}
& ERM \textit{(standard)}
& \metricci{.40}{.32}{.48}
& \metricci{.50}{.37}{.64}
& \metricci{.64}{.52}{.74}
& \metricci{.77}{.68}{.85}
& \metricci{.60}{.50}{.72}
& \metricci{.67}{.49}{.80}
& \metricci{.46}{.37}{.55}
& \secondmetricci{.77}{.66}{.86}
& \bestmetricci{.82}{.78}{.87}
& \metricci{.63}{.59}{.66} \\


& LS
& \metricci{.42}{.34}{.50}
& \secondmetricci{.57}{.44}{.70}
& \secondmetricci{.68}{.50}{.80}
& \metricci{.80}{.71}{.89}
& \metricci{.50}{.43}{.58}
& \secondmetricci{.74}{.61}{.86}
& \metricci{.53}{.43}{.62}
& \metricci{.71}{.57}{.83}
& \metricci{.72}{.60}{.81}
& \metricci{.63}{.59}{.67} \\


& ENN
& \secondmetricci{.47}{.42}{.52}
& \bestmetricci{.74}{.68}{.81}
& \metricci{.58}{.45}{.73}
& \bestmetricci{.85}{.76}{.92}
& \bestmetricci{.73}{.60}{.85}
& \metricci{.68}{.54}{.81}
& \bestmetricci{.81}{.72}{.89}
& \metricci{.74}{.60}{.84}
& \metricci{.78}{.74}{.82}
& \secondmetricci{.71}{.68}{.74} \\


& ERT \textit{(ours)}
& \bestmetricci{.63}{.54}{.71}
& \bestmetricci{.74}{.65}{.82}
& \bestmetricci{.71}{.53}{.84}
& \secondmetricci{.81}{.70}{.91}
& \secondmetricci{.65}{.42}{.84}
& \bestmetricci{.75}{.69}{.80}
& \secondmetricci{.79}{.71}{.87}
& \bestmetricci{.81}{.71}{.88}
& \secondmetricci{.81}{.77}{.84}
& \bestmetricci{.74}{.70}{.78} \\

\cmidrule{2-12}
& $\Delta$ vs.\ std.
& \sigposdelta{$+.23$}
& \sigposdelta{$+.24$}
& \posdelta{$+.07$}
& \posdelta{$+.05$}
& \posdelta{$+.04$}
& \posdelta{$+.08$}
& \sigposdelta{$+.33$}
& \posdelta{$+.03$}
& \negdelta{$-.02$}
& \sigposdelta{$+.12$} \\[-0.1em]

& $\Delta$ vs.\ best
& \sigposdelta{$+.16$}
& \neudelta{.00}
& \posdelta{$+.03$}
& \negdelta{$-.04$}
& \negdelta{$-.08$}
& \posdelta{$+.01$}
& \negdelta{$-.02$}
& \posdelta{$+.03$}
& \negdelta{$-.02$}
& \posdelta{$+.03$} \\
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{\footnotesize\editorlogo{claude}\,\textit{Claude Opus 5.5}}}
& ERM \textit{(standard)}
& \metricci{.41}{.29}{.52}
& \metricci{.33}{.21}{.46}
& \secondmetricci{.68}{.57}{.77}
& \metricci{.81}{.69}{.89}
& \metricci{.59}{.51}{.67}
& \metricci{.61}{.49}{.75}
& \metricci{.44}{.32}{.56}
& \secondmetricci{.72}{.59}{.83}
& \bestmetricci{.81}{.77}{.84}
& \metricci{.60}{.56}{.64} \\


& LS
& \metricci{.48}{.34}{.60}
& \metricci{.62}{.43}{.77}
& \bestmetricci{.80}{.77}{.85}
& \metricci{.81}{.59}{.94}
& \metricci{.48}{.36}{.60}
& \metricci{.64}{.58}{.70}
& \metricci{.51}{.39}{.62}
& \bestmetricci{.74}{.62}{.84}
& \metricci{.77}{.71}{.83}
& \metricci{.65}{.61}{.69} \\


& ENN
& \secondmetricci{.52}{.41}{.63}
& \bestmetricci{.79}{.71}{.86}
& \metricci{.66}{.59}{.73}
& \bestmetricci{.91}{.90}{.93}
& \secondmetricci{.60}{.47}{.72}
& \secondmetricci{.71}{.59}{.84}
& \secondmetricci{.60}{.50}{.71}
& \secondmetricci{.72}{.57}{.84}
& \metricci{.65}{.45}{.79}
& \secondmetricci{.68}{.65}{.72} \\


& ERT \textit{(ours)}
& \bestmetricci{.63}{.54}{.71}
& \secondmetricci{.76}{.68}{.83}
& \metricci{.67}{.52}{.80}
& \secondmetricci{.86}{.81}{.90}
& \bestmetricci{.61}{.46}{.73}
& \bestmetricci{.74}{.65}{.82}
& \bestmetricci{.74}{.63}{.83}
& \metricci{.70}{.55}{.83}
& \secondmetricci{.80}{.77}{.84}
& \bestmetricci{.72}{.69}{.76} \\

\cmidrule{2-12}
& $\Delta$ vs.\ std.
& \posdelta{$+.16$}
& \sigposdelta{$+.44$}
& \neudelta{.00}
& \posdelta{$+.05$}
& \posdelta{$+.02$}
& \sigposdelta{$+.12$}
& \sigposdelta{$+.30$}
& \negdelta{$-.02$}
& \negdelta{$-.01$}
& \sigposdelta{$+.12$} \\[-0.1em]

& $\Delta$ vs.\ best
& \sigposdelta{$+.10$}
& \negdelta{$-.02$}
& \negdelta{$-.13$}
& \negdelta{$-.05$}
& \posdelta{$+.01$}
& \posdelta{$+.03$}
& \posdelta{$+.14$}
& \negdelta{$-.04$}
& \negdelta{$-.01$}
& \posdelta{$+.04$} \\
\bottomrule
\end{tabular*}


==> ert-paper-arxiv/tables_bench/table1_open.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}c@{\hspace{3pt}}l*{9}{c}@{}}
\toprule
& & \multicolumn{4}{c}{\textbf{Relabel}} & \multicolumn{2}{c}{\textbf{Confusion fix}} & \multicolumn{2}{c}{\textbf{Subgroup fix}} & \\
\cmidrule(lr){3-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
 &
  & \textbf{WB}
  & \textbf{WB}
  & \textbf{C100}
  & \textbf{C100}
  & \textbf{C100}
  & \textbf{C100}
  & \textbf{PACS}
  & \textbf{PACS}
  & \\[-0.2em]
& \textbf{Method}
  & \textbf{R18}
  & \textbf{ViT}
  & \textbf{R18}
  & \textbf{ViT}
  & \textbf{R18}
  & \textbf{ViT}
  & \textbf{R18}
  & \textbf{ViT}
  & \textbf{Mean} \\
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{\footnotesize\editorlogo{glm}\,\textit{GLM-5.3-Flash}}}
& ERM \textit{(standard)}
& \bestmetricci{.44}{.28}{.59}
& \secondmetricci{.32}{.14}{.52}
& \metricci{.43}{.19}{.66}
& \bestmetricci{.66}{.42}{.85}
& \metricci{.69}{.56}{.79}
& \secondmetricci{.54}{.32}{.74}
& \metricci{.48}{.19}{.70}
& \bestmetricci{.44}{.22}{.65}
& \bestmetricci{.50}{.42}{.57} \\


& LS
& \metricci{.24}{.12}{.35}
& \metricci{.19}{.03}{.38}
& \secondmetricci{.59}{.36}{.78}
& \secondmetricci{.48}{.25}{.70}
& \metricci{.39}{.17}{.61}
& \metricci{.51}{.27}{.72}
& \secondmetricci{.56}{.29}{.76}
& \metricci{.07}{$-$.18}{.34}
& \metricci{.38}{.30}{.45} \\


& ENN
& \metricci{.30}{.15}{.46}
& \bestmetricci{.53}{.32}{.73}
& \metricci{.49}{.23}{.74}
& \metricci{.27}{.06}{.51}
& \bestmetricci{.76}{.60}{.88}
& \bestmetricci{.57}{.35}{.79}
& \metricci{.34}{.09}{.61}
& \metricci{.29}{.10}{.50}
& \metricci{.44}{.37}{.52} \\


& ERT \textit{(ours)}
& \secondmetricci{.38}{.18}{.58}
& \metricci{.24}{.03}{.48}
& \bestmetricci{.66}{.45}{.82}
& \metricci{.46}{.21}{.69}
& \secondmetricci{.73}{.50}{.88}
& \metricci{.46}{.21}{.71}
& \bestmetricci{.59}{.32}{.82}
& \secondmetricci{.42}{.22}{.59}
& \secondmetricci{.49}{.41}{.57} \\

\cmidrule{2-11}
& $\Delta$ vs.\ std.
& \negdelta{$-.06$}
& \negdelta{$-.08$}
& \posdelta{$+.22$}
& \negdelta{$-.20$}
& \posdelta{$+.03$}
& \negdelta{$-.08$}
& \posdelta{$+.12$}
& \negdelta{$-.02$}
& \negdelta{$-.01$} \\[-0.1em]

& $\Delta$ vs.\ best
& \negdelta{$-.06$}
& \negdelta{$-.29$}
& \posdelta{$+.07$}
& \negdelta{$-.20$}
& \negdelta{$-.03$}
& \negdelta{$-.11$}
& \posdelta{$+.04$}
& \negdelta{$-.02$}
& \negdelta{$-.01$} \\
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{\footnotesize\editorlogo{gemma}\,\textit{Gemma-4-26B}}}
& ERM \textit{(standard)}
& \metricci{.22}{.12}{.32}
& \secondmetricci{.17}{.07}{.29}
& \metricci{.34}{.10}{.63}
& \bestmetricci{.31}{.11}{.53}
& \metricci{.36}{.13}{.61}
& \bestmetricci{.47}{.24}{.69}
& \bestmetricci{.49}{.20}{.72}
& \metricci{.14}{.00}{.33}
& \secondmetricci{.31}{.24}{.39} \\


& LS
& \metricci{.18}{.08}{.30}
& \metricci{.11}{.05}{.20}
& \metricci{.25}{.05}{.51}
& \metricci{.00}{.00}{.01}
& \metricci{.29}{.08}{.58}
& \metricci{.27}{.06}{.53}
& \secondmetricci{.46}{.19}{.72}
& \metricci{.23}{.03}{.47}
& \metricci{.22}{.15}{.30} \\


& ENN
& \secondmetricci{.23}{.05}{.47}
& \metricci{.12}{.02}{.31}
& \bestmetricci{.40}{.12}{.69}
& \metricci{.15}{$-$.02}{.37}
& \secondmetricci{.41}{.11}{.71}
& \metricci{.39}{.05}{.72}
& \metricci{.34}{.10}{.59}
& \secondmetricci{.24}{.07}{.47}
& \metricci{.29}{.20}{.37} \\


& ERT \textit{(ours)}
& \bestmetricci{.30}{.13}{.50}
& \bestmetricci{.20}{.05}{.39}
& \secondmetricci{.39}{.10}{.68}
& \secondmetricci{.24}{.07}{.47}
& \bestmetricci{.64}{.33}{.87}
& \secondmetricci{.41}{.11}{.71}
& \metricci{.33}{.09}{.59}
& \bestmetricci{.46}{.19}{.70}
& \bestmetricci{.37}{.29}{.46} \\

\cmidrule{2-11}
& $\Delta$ vs.\ std.
& \posdelta{$+.09$}
& \posdelta{$+.03$}
& \posdelta{$+.05$}
& \negdelta{$-.07$}
& \posdelta{$+.28$}
& \negdelta{$-.06$}
& \negdelta{$-.16$}
& \posdelta{$+.32$}
& \posdelta{$+.06$} \\[-0.1em]

& $\Delta$ vs.\ best
& \posdelta{$+.07$}
& \posdelta{$+.03$}
& \negdelta{$-.01$}
& \negdelta{$-.07$}
& \posdelta{$+.23$}
& \negdelta{$-.06$}
& \negdelta{$-.16$}
& \posdelta{$+.22$}
& \posdelta{$+.06$} \\
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{\footnotesize\editorlogo{deepseek}\,\textit{DeepSeek-V4.1}}}
& ERM \textit{(standard)}
& \metricci{.42}{.28}{.55}
& \metricci{.49}{.32}{.64}
& \metricci{.74}{.67}{.79}
& \metricci{.86}{.80}{.89}
& \secondmetricci{.70}{.59}{.81}
& \bestmetricci{.74}{.57}{.89}
& \metricci{.65}{.46}{.80}
& \bestmetricci{.76}{.65}{.85}
& \secondmetricci{.67}{.62}{.71} \\


& LS
& \metricci{.42}{.27}{.56}
& \metricci{.49}{.26}{.71}
& \bestmetricci{.82}{.75}{.86}
& \bestmetricci{.92}{.91}{.93}
& \bestmetricci{.71}{.63}{.79}
& \secondmetricci{.70}{.57}{.83}
& \secondmetricci{.75}{.66}{.84}
& \bestmetricci{.76}{.68}{.83}
& \bestmetricci{.70}{.65}{.74} \\


& ENN
& \secondmetricci{.52}{.30}{.70}
& \bestmetricci{.75}{.66}{.82}
& \secondmetricci{.76}{.66}{.85}
& \metricci{.66}{.41}{.87}
& \metricci{.57}{.34}{.76}
& \metricci{.65}{.51}{.78}
& \metricci{.73}{.60}{.83}
& \metricci{.61}{.41}{.75}
& \metricci{.65}{.60}{.71} \\


& ERT \textit{(ours)}
& \bestmetricci{.64}{.45}{.78}
& \secondmetricci{.62}{.42}{.79}
& \metricci{.71}{.50}{.85}
& \secondmetricci{.90}{.88}{.93}
& \metricci{.66}{.45}{.81}
& \metricci{.62}{.49}{.75}
& \bestmetricci{.77}{.68}{.84}
& \secondmetricci{.64}{.50}{.76}
& \bestmetricci{.70}{.64}{.75} \\

\cmidrule{2-11}
& $\Delta$ vs.\ std.
& \sigposdelta{$+.23$}
& \posdelta{$+.14$}
& \negdelta{$-.02$}
& \posdelta{$+.05$}
& \negdelta{$-.04$}
& \negdelta{$-.12$}
& \posdelta{$+.12$}
& \negdelta{$-.12$}
& \posdelta{$+.03$} \\[-0.1em]

& $\Delta$ vs.\ best
& \posdelta{$+.13$}
& \negdelta{$-.13$}
& \negdelta{$-.10$}
& \negdelta{$-.02$}
& \negdelta{$-.05$}
& \negdelta{$-.12$}
& \posdelta{$+.02$}
& \negdelta{$-.12$}
& \neudelta{.00} \\
\bottomrule
\end{tabular*}


==> ert-paper-arxiv/tables_bench/tests_astra.tex <==
Waterbirds relabel, ResNet-18 & $+0.01$ & 4/8 & 0.719 & $+0.06$ & 7/8 & 0.195 & $+0.23$ & 8/8 & 0.008 \\
Waterbirds relabel, ViT-B/16 & $+0.06$ & 6/8 & 0.391 & $+0.23$ & 7/8 & 0.039 & $+0.24$ & 7/8 & 0.016 \\
CIFAR-100 relabel, ResNet-18 & $+0.04$ & 4/8 & 0.578 & $-0.05$ & 3/8 & 0.523 & $+0.07$ & 5/8 & 0.438 \\
CIFAR-100 relabel, ViT-B/16 & $+0.03$ & 6/8 & 0.516 & $+0.09$ & 7/8 & 0.062 & $+0.05$ & 5/8 & 0.391 \\
CIFAR-100 confusion fix, ResNet-18 & $-0.10$ & 1/8 & 0.031 & $+0.13$ & 5/8 & 0.164 & $+0.04$ & 5/8 & 0.648 \\
CIFAR-100 confusion fix, ViT-B/16 & $+0.07$ & 6/8 & 0.500 & $+0.01$ & 5/8 & 0.945 & $+0.08$ & 5/8 & 0.336 \\
Entity-30 confusion fix, ResNet-50 & $+0.07$ & 6/9 & 0.406 & $+0.36$ & 9/9 & 0.004 & $+0.33$ & 9/9 & 0.004 \\
PACS subgroup fix, ResNet-18 & $-0.06$ & 2/8 & 0.062 & $-0.04$ & 3/8 & 0.219 & $+0.03$ & 5/8 & 0.188 \\
PACS subgroup fix, ViT-B/16 & $-0.11$ & 0/8 & 0.008 & $-0.04$ & 2/8 & 0.148 & $-0.02$ & 3/8 & 0.586 \\


==> ert-paper-arxiv/tables_bench/tests_opus.tex <==
Waterbirds relabel, ResNet-18 & $+0.07$ & 5/8 & 0.336 & $+0.09$ & 4/8 & 0.531 & $+0.16$ & 5/8 & 0.133 \\
Waterbirds relabel, ViT-B/16 & $+0.29$ & 6/8 & 0.031 & $+0.46$ & 8/8 & 0.008 & $+0.44$ & 8/8 & 0.008 \\
CIFAR-100 relabel, ResNet-18 & $+0.13$ & 7/8 & 0.023 & $-0.02$ & 4/8 & 0.695 & $-0.00$ & 4/8 & 0.953 \\
CIFAR-100 relabel, ViT-B/16 & $+0.00$ & 6/8 & 1.000 & $+0.10$ & 8/8 & 0.008 & $+0.05$ & 4/8 & 0.508 \\
CIFAR-100 confusion fix, ResNet-18 & $-0.11$ & 2/8 & 0.227 & $+0.01$ & 4/8 & 0.883 & $+0.02$ & 4/8 & 0.844 \\
CIFAR-100 confusion fix, ViT-B/16 & $+0.02$ & 5/8 & 0.805 & $+0.10$ & 6/8 & 0.078 & $+0.12$ & 7/8 & 0.023 \\
Entity-30 confusion fix, ResNet-50 & $+0.08$ & 7/9 & 0.523 & $+0.16$ & 7/9 & 0.027 & $+0.30$ & 8/9 & 0.027 \\
PACS subgroup fix, ResNet-18 & $+0.02$ & 4/8 & 0.383 & $-0.00$ & 4/8 & 0.922 & $-0.02$ & 3/8 & 0.500 \\
PACS subgroup fix, ViT-B/16 & $-0.04$ & 4/8 & 0.312 & $-0.16$ & 0/8 & 0.008 & $-0.01$ & 3/8 & 0.734 \\


==> tables_bench/ablation_edits.tex <==
\begin{tabular}{@{}lcccc@{}}
\toprule
Rehearsed edit & Net & $\Delta$ & Pairs $>0$ & $p$ \\
\midrule
\multicolumn{5}{@{}l}{\emph{One training seed, 8 species}} \\
ERT (reference) & 0.72 & & & \\
\quad + bias compensation & 0.76 & $+0.04$ & 4/8 & 0.55 \\
\quad 32 units instead of 8 & 0.76 & $+0.03$ & 4/8 & 0.51 \\
\quad 8 to 64 units, drawn per episode & 0.68 & $-0.04$ & 2/8 & 0.62 \\
\quad step size $\times$1 to 3 & 0.66 & $-0.06$ & 2/8 & 0.26 \\
\quad + agent-shaped edits, combined & 0.75 & $+0.02$ & 3/8 & 0.62 \\
\midrule
\multicolumn{5}{@{}l}{\emph{Two training seeds, 16 pairs}} \\
ERT (reference) & 0.68 & & & \\
\quad stronger rehearsal & 0.73 & $+0.06$ & 10/16 & 0.20 \\
\quad + gradient-step edit & 0.69 & $+0.01$ & 9/16 & 0.79 \\
\bottomrule
\end{tabular}


==> tables_bench/ablation_edits_settings.tex <==
\begin{tabular}{@{}lllccccc@{}}
\toprule
Task & Dataset & Network & Pairs & ERT & Variant & $\Delta$ & $p$ \\
\midrule
\multicolumn{8}{@{}l}{\emph{Stronger rehearsal (16 episodes, 64 units, two support images)}} \\
Relabel & Waterbirds & ResNet-18 & 16 & 0.68 & 0.73 & $+0.06$ & 0.20 \\
Relabel & Waterbirds & ViT-B/16 & 8 & 0.82 & 0.76 & $-0.06$ & 0.38 \\
Relabel & CIFAR-100 & ResNet-18 & 8 & 0.67 & 0.61 & $-0.07$ & 0.47 \\
Relabel & CIFAR-100 & ViT-B/16 & 8 & 0.86 & 0.88 & $+0.02$ & 0.58 \\
Confusion fix & CIFAR-100 & ResNet-18 & 8 & 0.61 & 0.51 & $-0.10$ & 0.20 \\
Confusion fix & CIFAR-100 & ViT-B/16 & 8 & 0.74 & 0.69 & $-0.05$ & 0.76 \\
Subgroup fix & PACS & ResNet-18 & 8 & 0.70 & 0.77 & $+0.07$ & 0.02 \\
Subgroup fix & PACS & ViT-B/16 & 8 & 0.80 & 0.66 & $-0.14$ & 0.13 \\
\multicolumn{6}{@{}l}{Mean over settings} & $-0.03$ & \\
\midrule
\multicolumn{8}{@{}l}{\emph{Signed sparse edit instead of the top-8 rule}} \\
Relabel & Waterbirds & ViT-B/16 & 8 & 0.82 & 0.81 & $-0.01$ & 0.75 \\
Relabel & CIFAR-100 & ViT-B/16 & 8 & 0.86 & 0.89 & $+0.03$ & 0.34 \\
\bottomrule
\end{tabular}


==> tables_bench/detail_opus.tex <==
Waterbirds relabel, ResNet-18 & 0.51 & 0.101 & $-5.1$ & 87.5 & 0.62 & 0.144 & $-6.0$ & 84.7 & 0.63 & 0.109 & $-7.0$ & 91.4 & 0.73 & 0.107 & $-6.3$ & 91.4 \\
Waterbirds relabel, ViT-B/16 & 0.39 & 0.059 & $-3.8$ & 87.5 & 0.72 & 0.099 & $-5.5$ & 89.1 & 0.87 & 0.081 & $-5.6$ & 93.2 & 0.85 & 0.085 & $-6.5$ & 93.2 \\
CIFAR-100 relabel, ResNet-18 & 0.71 & 0.035 & $-2.8$ & 86.9 & 0.85 & 0.050 & $-4.0$ & 87.6 & 0.71 & 0.050 & $-4.2$ & 87.4 & 0.72 & 0.046 & $-4.0$ & 85.7 \\
CIFAR-100 relabel, ViT-B/16 & 0.84 & 0.029 & $-3.0$ & 93.1 & 0.84 & 0.027 & $-3.1$ & 93.4 & 0.94 & 0.027 & $-3.2$ & 93.5 & 0.88 & 0.020 & $-2.4$ & 93.0 \\
CIFAR-100 confusion fix, ResNet-18 & 0.61 & 0.014 & $-0.8$ & 86.9 & 0.50 & 0.016 & $-1.1$ & 87.7 & 0.63 & 0.026 & $-1.8$ & 87.4 & 0.64 & 0.024 & $-1.5$ & 85.7 \\
CIFAR-100 confusion fix, ViT-B/16 & 0.62 & 0.004 & $-0.2$ & -- & 0.64 & 0.006 & $-0.3$ & -- & 0.72 & 0.006 & $-0.4$ & -- & 0.74 & 0.005 & $-0.2$ & -- \\
Entity-30 confusion fix, ResNet-50 & 0.45 & 0.014 & $-1.0$ & 91.2 & 0.53 & 0.019 & $-1.9$ & 91.5 & 0.61 & 0.015 & $-1.0$ & 91.2 & 0.77 & 0.032 & $-2.4$ & 90.7 \\
PACS subgroup fix, ResNet-18 & 0.78 & 0.057 & $-3.4$ & 88.6 & 0.82 & 0.081 & $-5.1$ & 88.3 & 0.83 & 0.110 & $-7.2$ & 86.9 & 0.79 & 0.088 & $-5.4$ & 86.9 \\
PACS subgroup fix, ViT-B/16 & 0.88 & 0.070 & $-4.1$ & 90.0 & 0.84 & 0.069 & $-4.1$ & 90.0 & 0.71 & 0.063 & $-3.8$ & 89.0 & 0.91 & 0.110 & $-6.6$ & 85.0 \\


==> tables_bench/edit_heatmap_stats.tex <==
\begin{tabular}{@{}l rr rrr rrr rrr r@{}}
\toprule
 & & & \multicolumn{3}{c}{Edited units} & \multicolumn{3}{c}{Change of a unit} & \multicolumn{3}{c}{Change of the head} & \\
\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}
 & Edits & Head & min & mean & max & min & mean & max & min & mean & max & Outside \\
\midrule
\multicolumn{13}{@{}l}{\emph{ResNet-18} (512 units)} \\
\quad Opus & 144 & 142 & 1 & 20 & 75 & $2\cdot10^{-7}$ & 0.39 & 22.1 & 0.19 & 2.15 & 22.2 & 13 \\
\quad Astra & 128 & 128 & 1 & 206 & 512 & $1\cdot10^{-7}$ & 0.05 & 10.2 & 0.13 & 1.53 & 17.7 & 4 \\
\quad Gemma & 125 & 63 & 1 & 47 & 512 & $2\cdot10^{-6}$ & 0.16 & 7.07 & 0.08 & 1.98 & 10.1 & 1 \\
\quad GLM & 126 & 107 & 1 & 37 & 512 & $2\cdot10^{-7}$ & 0.12 & 8.00 & $9\cdot10^{-5}$ & 1.14 & 11.3 & 3 \\
\quad DeepSeek & 119 & 118 & 3 & 35 & 94 & $5\cdot10^{-7}$ & 0.12 & 2.00 & 0.09 & 0.85 & 6.82 & 0 \\
\quad all editors & 642 & 558 & 1 & 72 & 512 & $1\cdot10^{-7}$ & 0.10 & 22.1 & $9\cdot10^{-5}$ & 1.52 & 22.2 & 21 \\
\midrule
\multicolumn{13}{@{}l}{\emph{ResNet-50} (2048 units)} \\
\quad Opus & 36 & 33 & 8 & 36 & 142 & $1\cdot10^{-7}$ & 1.43 & 15.1 & 2.51 & 9.97 & 39.0 & 0 \\
\quad Astra & 36 & 35 & 1 & 373 & 2048 & $6\cdot10^{-6}$ & 0.21 & 400 & 0.74 & 21.6 & 400 & 0 \\
\quad all editors & 72 & 68 & 1 & 210 & 2048 & $1\cdot10^{-7}$ & 0.31 & 400 & 0.74 & 15.9 & 400 & 0 \\
\midrule
\multicolumn{13}{@{}l}{\emph{ViT} (768 units)} \\
\quad Opus & 128 & 121 & 2 & 71 & 768 & $3\cdot10^{-5}$ & 0.13 & 2.50 & 0.31 & 1.50 & 7.03 & 1 \\
\quad Astra & 128 & 128 & 51 & 638 & 768 & $2\cdot10^{-7}$ & 0.03 & 1.01 & 0.18 & 0.98 & 3.55 & 0 \\
\quad Gemma & 126 & 52 & 1 & 300 & 768 & $1\cdot10^{-5}$ & 8.65 & 653 & 0.38 & 116 & 5693 & 0 \\
\quad GLM & 125 & 87 & 1 & 127 & 768 & $2\cdot10^{-5}$ & 0.15 & 39.7 & 0.09 & 3.61 & 39.7 & 3 \\
\quad DeepSeek & 126 & 100 & 11 & 122 & 768 & $3\cdot10^{-6}$ & 0.11 & 4.81 & 0.18 & 1.66 & 16.0 & 0 \\
\quad all editors & 633 & 488 & 1 & 265 & 768 & $2\cdot10^{-7}$ & 1.09 & 653 & 0.09 & 14.0 & 5693 & 4 \\
\midrule
\multicolumn{13}{@{}l}{\emph{Training method} (all backbones and editors)} \\
\quad ERM & 335 & 284 & 1 & 165 & 768 & $1\cdot10^{-7}$ & 0.12 & 22.1 & 0.15 & 3.04 & 24.3 & 7 \\
\quad LS & 333 & 270 & 1 & 166 & 768 & $2\cdot10^{-7}$ & 0.06 & 5.32 & 0.06 & 1.28 & 14.0 & 5 \\
\quad ENN & 340 & 279 & 1 & 165 & 2048 & $5\cdot10^{-7}$ & 2.91 & 653 & 0.12 & 22.4 & 5693 & 10 \\
\quad ERT & 339 & 281 & 1 & 164 & 2048 & $2\cdot10^{-6}$ & 0.17 & 400 & $9\cdot10^{-5}$ & 4.67 & 400 & 3 \\
\bottomrule
\end{tabular}


==> tables_bench/ert_vs_enn.tex <==
Waterbirds relabel, ResNet-18 & $+0.10$ & 10/16 & 0.043 \\
Waterbirds relabel, ViT-B/16 & $-0.02$ & 4/8 & 0.414 \\
CIFAR-100 relabel, ResNet-18 & $+0.02$ & 4/8 & 0.805 \\
CIFAR-100 relabel, ViT-B/16 & $-0.05$ & 2/8 & 0.062 \\
CIFAR-100 confusion fix, ResNet-18 & $+0.01$ & 5/8 & 0.820 \\
CIFAR-100 confusion fix, ViT-B/16 & $+0.03$ & 4/8 & 0.719 \\
Entity-30 confusion fix, ResNet-50 & $+0.14$ & 7/9 & 0.227 \\
PACS subgroup fix, ResNet-18 & $-0.01$ & 4/8 & 0.812 \\
PACS subgroup fix, ViT-B/16 & $+0.15$ & 7/8 & 0.078 \\


==> tables_bench/table1_open.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}c@{\hspace{3pt}}l*{9}{c}@{}}
\toprule
& & \multicolumn{4}{c}{\textbf{Relabel}} & \multicolumn{2}{c}{\textbf{Confusion fix}} & \multicolumn{2}{c}{\textbf{Subgroup fix}} & \\
\cmidrule(lr){3-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}
 &
  & \textbf{WB}
  & \textbf{WB}
  & \textbf{C100}
  & \textbf{C100}
  & \textbf{C100}
  & \textbf{C100}
  & \textbf{PACS}
  & \textbf{PACS}
  & \\[-0.2em]
& \textbf{Method}
  & \textbf{R18}
  & \textbf{ViT}
  & \textbf{R18}
  & \textbf{ViT}
  & \textbf{R18}
  & \textbf{ViT}
  & \textbf{R18}
  & \textbf{ViT}
  & \textbf{Mean} \\
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{\footnotesize\editorlogo{glm}\,\textit{GLM-5.3-Flash}}}
& ERM \textit{(standard)}
& \bestmetricci{.44}{.28}{.59}
& \secondmetricci{.32}{.14}{.52}
& \metricci{.43}{.19}{.66}
& \bestmetricci{.66}{.42}{.85}
& \metricci{.69}{.56}{.79}
& \secondmetricci{.54}{.32}{.74}
& \metricci{.48}{.19}{.70}
& \bestmetricci{.44}{.22}{.65}
& \bestmetricci{.50}{.42}{.57} \\


& LS
& \metricci{.24}{.12}{.35}
& \metricci{.19}{.03}{.38}
& \secondmetricci{.59}{.36}{.78}
& \secondmetricci{.48}{.25}{.70}
& \metricci{.39}{.17}{.61}
& \metricci{.51}{.27}{.72}
& \secondmetricci{.56}{.29}{.76}
& \metricci{.07}{$-$.18}{.34}
& \metricci{.38}{.30}{.45} \\


& ENN
& \metricci{.30}{.15}{.46}
& \bestmetricci{.53}{.32}{.73}
& \metricci{.49}{.23}{.74}
& \metricci{.27}{.06}{.51}
& \bestmetricci{.76}{.60}{.88}
& \bestmetricci{.57}{.35}{.79}
& \metricci{.34}{.09}{.61}
& \metricci{.29}{.10}{.50}
& \metricci{.44}{.37}{.52} \\


& ERT \textit{(ours)}
& \secondmetricci{.38}{.18}{.58}
& \metricci{.24}{.03}{.48}
& \bestmetricci{.66}{.45}{.82}
& \metricci{.46}{.21}{.69}
& \secondmetricci{.73}{.50}{.88}
& \metricci{.46}{.21}{.71}
& \bestmetricci{.59}{.32}{.82}
& \secondmetricci{.42}{.22}{.59}
& \secondmetricci{.49}{.41}{.57} \\

\cmidrule{2-11}
& $\Delta$ vs.\ std.
& \negdelta{$-.06$}
& \negdelta{$-.08$}
& \posdelta{$+.22$}
& \negdelta{$-.20$}
& \posdelta{$+.03$}
& \negdelta{$-.08$}
& \posdelta{$+.12$}
& \negdelta{$-.02$}
& \negdelta{$-.01$} \\[-0.1em]

& $\Delta$ vs.\ best
& \negdelta{$-.06$}
& \negdelta{$-.29$}
& \posdelta{$+.07$}
& \negdelta{$-.20$}
& \negdelta{$-.03$}
& \negdelta{$-.11$}
& \posdelta{$+.04$}
& \negdelta{$-.02$}
& \negdelta{$-.01$} \\
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{\footnotesize\editorlogo{gemma}\,\textit{Gemma-4-26B}}}
& ERM \textit{(standard)}
& \metricci{.22}{.12}{.32}
& \secondmetricci{.17}{.07}{.29}
& \metricci{.34}{.10}{.63}
& \bestmetricci{.31}{.11}{.53}
& \metricci{.36}{.13}{.61}
& \bestmetricci{.47}{.24}{.69}
& \bestmetricci{.49}{.20}{.72}
& \metricci{.14}{.00}{.33}
& \secondmetricci{.31}{.24}{.39} \\


& LS
& \metricci{.18}{.08}{.30}
& \metricci{.11}{.05}{.20}
& \metricci{.25}{.05}{.51}
& \metricci{.00}{.00}{.01}
& \metricci{.29}{.08}{.58}
& \metricci{.27}{.06}{.53}
& \secondmetricci{.46}{.19}{.72}
& \metricci{.23}{.03}{.47}
& \metricci{.22}{.15}{.30} \\


& ENN
& \secondmetricci{.23}{.05}{.47}
& \metricci{.12}{.02}{.31}
& \bestmetricci{.40}{.12}{.69}
& \metricci{.15}{$-$.02}{.37}
& \secondmetricci{.41}{.11}{.71}
& \metricci{.39}{.05}{.72}
& \metricci{.34}{.10}{.59}
& \secondmetricci{.24}{.07}{.47}
& \metricci{.29}{.20}{.37} \\


& ERT \textit{(ours)}
& \bestmetricci{.30}{.13}{.50}
& \bestmetricci{.20}{.05}{.39}
& \secondmetricci{.39}{.10}{.68}
& \secondmetricci{.24}{.07}{.47}
& \bestmetricci{.64}{.33}{.87}
& \secondmetricci{.41}{.11}{.71}
& \metricci{.33}{.09}{.59}
& \bestmetricci{.46}{.19}{.70}
& \bestmetricci{.37}{.29}{.46} \\

\cmidrule{2-11}
& $\Delta$ vs.\ std.
& \posdelta{$+.09$}
& \posdelta{$+.03$}
& \posdelta{$+.05$}
& \negdelta{$-.07$}
& \posdelta{$+.28$}
& \negdelta{$-.06$}
& \negdelta{$-.16$}
& \posdelta{$+.32$}
& \posdelta{$+.06$} \\[-0.1em]

& $\Delta$ vs.\ best
& \posdelta{$+.07$}
& \posdelta{$+.03$}
& \negdelta{$-.01$}
& \negdelta{$-.07$}
& \posdelta{$+.23$}
& \negdelta{$-.06$}
& \negdelta{$-.16$}
& \posdelta{$+.22$}
& \posdelta{$+.06$} \\
\midrule
\multirow{6}{*}{\rotatebox[origin=c]{90}{\footnotesize\editorlogo{deepseek}\,\textit{DeepSeek-V4.1}}}
& ERM \textit{(standard)}
& \metricci{.42}{.28}{.55}
& \metricci{.49}{.32}{.64}
& \metricci{.74}{.67}{.79}
& \metricci{.86}{.80}{.89}
& \secondmetricci{.70}{.59}{.81}
& \bestmetricci{.74}{.57}{.89}
& \metricci{.65}{.46}{.80}
& \bestmetricci{.76}{.65}{.85}
& \secondmetricci{.67}{.62}{.71} \\


& LS
& \metricci{.42}{.27}{.56}
& \metricci{.49}{.26}{.71}
& \bestmetricci{.82}{.75}{.86}
& \bestmetricci{.92}{.91}{.93}
& \bestmetricci{.71}{.63}{.79}
& \secondmetricci{.70}{.57}{.83}
& \secondmetricci{.75}{.66}{.84}
& \bestmetricci{.76}{.68}{.83}
& \bestmetricci{.70}{.65}{.74} \\


& ENN
& \secondmetricci{.52}{.30}{.70}
& \bestmetricci{.75}{.66}{.82}
& \secondmetricci{.76}{.66}{.85}
& \metricci{.66}{.41}{.87}
& \metricci{.57}{.34}{.76}
& \metricci{.65}{.51}{.78}
& \metricci{.73}{.60}{.83}
& \metricci{.61}{.41}{.75}
& \metricci{.65}{.60}{.71} \\


& ERT \textit{(ours)}
& \bestmetricci{.64}{.45}{.78}
& \secondmetricci{.62}{.42}{.79}
& \metricci{.71}{.50}{.85}
& \secondmetricci{.90}{.88}{.93}
& \metricci{.66}{.45}{.81}
& \metricci{.62}{.49}{.75}
& \bestmetricci{.77}{.68}{.84}
& \secondmetricci{.64}{.50}{.76}
& \bestmetricci{.70}{.64}{.75} \\

\cmidrule{2-11}
& $\Delta$ vs.\ std.
& \sigposdelta{$+.23$}
& \posdelta{$+.14$}
& \negdelta{$-.02$}
& \posdelta{$+.05$}
& \negdelta{$-.04$}
& \negdelta{$-.12$}
& \posdelta{$+.12$}
& \negdelta{$-.12$}
& \posdelta{$+.03$} \\[-0.1em]

& $\Delta$ vs.\ best
& \posdelta{$+.13$}
& \negdelta{$-.13$}
& \negdelta{$-.10$}
& \negdelta{$-.02$}
& \negdelta{$-.05$}
& \negdelta{$-.12$}
& \posdelta{$+.02$}
& \negdelta{$-.12$}
& \neudelta{.00} \\
\bottomrule
\end{tabular*}


==> tables_bench/tests_astra.tex <==
Waterbirds relabel, ResNet-18 & $+0.01$ & 4/8 & 0.719 & $+0.06$ & 7/8 & 0.195 & $+0.23$ & 8/8 & 0.008 \\
Waterbirds relabel, ViT-B/16 & $+0.06$ & 6/8 & 0.391 & $+0.23$ & 7/8 & 0.039 & $+0.24$ & 7/8 & 0.016 \\
CIFAR-100 relabel, ResNet-18 & $+0.04$ & 4/8 & 0.578 & $-0.05$ & 3/8 & 0.523 & $+0.07$ & 5/8 & 0.438 \\
CIFAR-100 relabel, ViT-B/16 & $+0.03$ & 6/8 & 0.516 & $+0.09$ & 7/8 & 0.062 & $+0.05$ & 5/8 & 0.391 \\
CIFAR-100 confusion fix, ResNet-18 & $-0.10$ & 1/8 & 0.031 & $+0.13$ & 5/8 & 0.164 & $+0.04$ & 5/8 & 0.648 \\
CIFAR-100 confusion fix, ViT-B/16 & $+0.07$ & 6/8 & 0.500 & $+0.01$ & 5/8 & 0.945 & $+0.08$ & 5/8 & 0.336 \\
Entity-30 confusion fix, ResNet-50 & $+0.07$ & 6/9 & 0.406 & $+0.36$ & 9/9 & 0.004 & $+0.33$ & 9/9 & 0.004 \\
PACS subgroup fix, ResNet-18 & $-0.06$ & 2/8 & 0.062 & $-0.04$ & 3/8 & 0.219 & $+0.03$ & 5/8 & 0.188 \\
PACS subgroup fix, ViT-B/16 & $-0.11$ & 0/8 & 0.008 & $-0.04$ & 2/8 & 0.148 & $-0.02$ & 3/8 & 0.586 \\


==> tables_bench/tests_opus.tex <==
Waterbirds relabel, ResNet-18 & $+0.07$ & 5/8 & 0.336 & $+0.09$ & 4/8 & 0.531 & $+0.16$ & 5/8 & 0.133 \\
Waterbirds relabel, ViT-B/16 & $+0.29$ & 6/8 & 0.031 & $+0.46$ & 8/8 & 0.008 & $+0.44$ & 8/8 & 0.008 \\
CIFAR-100 relabel, ResNet-18 & $+0.13$ & 7/8 & 0.023 & $-0.02$ & 4/8 & 0.695 & $-0.00$ & 4/8 & 0.953 \\
CIFAR-100 relabel, ViT-B/16 & $+0.00$ & 6/8 & 1.000 & $+0.10$ & 8/8 & 0.008 & $+0.05$ & 4/8 & 0.508 \\
CIFAR-100 confusion fix, ResNet-18 & $-0.11$ & 2/8 & 0.227 & $+0.01$ & 4/8 & 0.883 & $+0.02$ & 4/8 & 0.844 \\
CIFAR-100 confusion fix, ViT-B/16 & $+0.02$ & 5/8 & 0.805 & $+0.10$ & 6/8 & 0.078 & $+0.12$ & 7/8 & 0.023 \\
Entity-30 confusion fix, ResNet-50 & $+0.08$ & 7/9 & 0.523 & $+0.16$ & 7/9 & 0.027 & $+0.30$ & 8/9 & 0.027 \\
PACS subgroup fix, ResNet-18 & $+0.02$ & 4/8 & 0.383 & $-0.00$ & 4/8 & 0.922 & $-0.02$ & 3/8 & 0.500 \\
PACS subgroup fix, ViT-B/16 & $-0.04$ & 4/8 & 0.312 & $-0.16$ & 0/8 & 0.008 & $-0.01$ & 3/8 & 0.734 \\

